The Anatomy of Large-Scale Distributed Graph Algorithms

The increasing complexity of the software/hardware stack of modern supercomputers results in explosion of parameters. The performance analysis becomes a truly experimental science, even more challenging in the presence of massive irregularity and data dependency. We analyze how the existing body of research handles the experimental aspect in the context of distributed graph algorithms (DGAs). We distinguish algorithm-level contributions, often prioritized by authors, from runtime-level concerns that are harder to place. We show that the runtime is such an integral part of DGAs that experimental results are difficult to interpret and extrapolate without understanding the properties of the runtime used. We argue that in order to gain understanding about the impact of runtimes, more information needs to be gathered. To begin this process, we provide an initial set of recommendations for describing DGA results based on our analysis of the current state of the field.

==> README <==
cleveref, a LaTeX package for intelligent cross-referencing
Copyright (C) 2007--2013  Toby Cubitt

Files:
cleveref.ins  Batch file, run through LaTeX
cleveref.dtx  Docstrip archive, run through LaTeX
cleveref.sty  LaTeX package, generated by cleveref.ins from cleveref.dtx
cleveref.dvi  Package documentation, generated from cleveref.dtx
cleveref.pdf  Package documentation; can also be generated from cleveref.dtx
README        This file

E-mail:   toby-cleveref@dr-qubit.org
Address:  DAMTP, University of Cambridge, United Kingdom

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


Description:
------------
The cleveref package enhances LaTeX's cross-referencing features, allowing the
format of cross-references to be determined automatically according to the
"type" of cross-reference (equation, section, etc.) and the context in which
the cross-reference is used. The formatting for each cross-reference type can
be fully customised in the preamble of your document. In addition, cleveref
can type-set cross-references to lists of multiple labels, automatically
formatting them according to their types, sorting them, and compressing
sequences of numerically consecutive labels. Again, the multiple-reference
formatting is fully customisable. Though a number of other packages provide
similar features, all have certain deficiencies which cleveref attempts to
overcome.

Using cleveref is easy. Basically, wherever you would previously have used
\ref, you can use \cref instead. (Except at the beginning of a sentence, where
you should use \Cref.)  You no longer need to put the name of the thing you're
referencing in front of the \cref command, because cleveref will sort that out
for you: i.e. use "\cref{eq1}" instead of "eq.~(\ref{eq1})". If you want to
refer to a range of labels, use the \crefrange command: "\crefrange{eq1}{eq5}"
produces "eqs.~(1) to~(5)". Finally, if you want to refer to multiple things
at once, you can now combine them all into one cross-reference and leave
cleveref to sort it out: e.g. "\cref{eq2,eq1,eq3,eq5,thm2,def1}" produces:
"eqs.~(1) to~(3) and~(5), theorem~5, and definition~1".

Cleveref has various other useful features. For details, see the package
documentation.


==> editingmarks.tex <==


\usepackage{color}

% For SC:
\newcommand{\eh}[1]{\pgwrapper{ETH}{#1}}
\newcommand{\eric}[1]{\eh{#1}}


%\InputIfFileExists{activateeditingmarks}{
%}{
%    \def\noeditingmarks{}
%}

\definecolor{comment-red}{rgb}{0.8,0,0}
\ifx\noeditingmarks\undefined
   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}
   \newcommand{\auditme}[1]{{\color{comment-red}{#1}}}
   \newcommand{\pgwrapper}[2]{\textred{(#1: #2)}}
   \newcommand{\note}[1]{{\begin{itemize}\item \textcolor{blue}{#1} \end{itemize}}}
   \newcommand{\new}[1]{{\color{darkgreen}{#1}}}
   \newcommand{\const}[1]{\textred{#1}}
   \newcommand{\Red}[1]{{\color{comment-red}{#1}}}

\else
%   \newcommand{\textred}[1]{#1}
%   \newcommand{\auditme}[1]{#1}
   \newcommand{\auditme}[1]{{\color{comment-red}{#1}}}
   \newcommand{\textred}[1]{{\color{comment-red}{#1}}}
   \newcommand{\pgwrapper}[2]{}
%   \newcommand{\note}[1]{}
   \newcommand{\note}[1]{{\begin{itemize}\item \textcolor{blue}{#1} \end{itemize}}}
   \newcommand{\new}[1]{#1}
%   \newcommand{\new}[1]{\textcolor{blue}{#1}}
   \newcommand{\const}[1]{#1}
\fi

\newcommand{\todo}[1]{\note{#1}}

